Measuring Wigner functions of quantum states of light in the undergraduate laboratory

In this work, we present an educational activity aimed at measuring the Wigner distribution functions of quantum states of light in the undergraduate laboratory. This project was conceived by students from various courses within the physics undergraduate curriculum, and its outcomes were used in an introductory Quantum Optics course at the Universidad de los Andes in Bogot\'a, Colombia. The activity entails a two-hour laboratory practice in which students engage with a pre-aligned experimental setup. They subsequently employ an open-access, custom-made computational graphical user interface to reconstruct the Wigner distribution function for various quantum states of light. Given that the testing phase coincided with the COVID-19 pandemic, we incorporated the capacity to analyze simulated data into the computational user interface. The activity is now part of the course syllabus and its virtual component has proven to be highly valuable for the implementation of distance learning in quantum optics.

==> Figures/PhaseSpaceCoh.tex <==
\begin{tikzpicture}
    \begin{scope}[thick,font=\scriptsize,scale=2]
    % Axes:
    % Are simply drawn using line with the `->` option to make them arrows:
    % The main labels of the axes can be places using `node`s:

    \begin{scope}[scale=0.7,yshift=1cm]
    \begin{scope}[xshift=0.4cm,yshift=0.4cm,rotate=-45,scale=1.5]
    \draw[color=red!60, fill=red!10, very thick](0,0) ellipse (0.2 and 0.05);
        \draw[-,red,thin,dotted] (-0.2,-0.05) -- (-0.2,0.05);
    \draw[-,red,thin,dotted] (-0.2,0.05) -- (0.2,0.05);
    
    \draw[-,red,thin,dotted] (0.2,-0.05) -- (0.2,0.05);
    \draw[-,red,thin,dotted] (-0.2,-0.05) -- (0.2,-0.05);

    
    \end{scope}
    
    \draw [->] (-0.5,0) -- (0.7,0) node [right]  {$x$};
    \draw [->] (0,-0.2) -- (0,0.7) node [above] {$p$};
    
    \draw [->,red] (0,0) -- (0.4cm,0.4cm);
    
    \draw[red,semitransparent] (0.25,0) arc (0:45:0.25) node[yshift=-0.8,right,font=\scriptsize]{$\phi$};
      
          \end{scope}
          \end{scope}
   

\end{tikzpicture}
